PAC Statistical Model Checking for Markov Decision Processes and Stochastic Games

Statistical model checking (SMC) is a technique for analysis of probabilistic systems that may be (partially) unknown. We present an SMC algorithm for (unbounded) reachability yielding probably approximately correct (PAC) guarantees on the results. We consider both the setting (i) with no knowledge of the transition function (with the only quantity required a bound on the minimum transition probability) and (ii) with knowledge of the topology of the underlying graph. On the one hand, it is the first algorithm for stochastic games. On the other hand, it is the first practical algorithm even for Markov decision processes. Compared to previous approaches where PAC guarantees require running times longer than the age of universe even for systems with a handful of states, our algorithm often yields reasonably precise results within minutes, not requiring the knowledge of mixing time or the topology of the whole model.

==> dump.tex <==
\section{Main Content}

%Probably later in its own file, maybe even own section
\subsection{DQL for Markov Decision Processes and Stochastic Games}
Also: Use structure, \cite{DHKP16} trick: This is a different version of $\EXPLOREBREAK$. For $\EXPLOREBREAK$, we have: immediately when seeing state twice, path longer than $c \cdot \abs{\Vis}$ or candidate detection from \cite{DHKP16}.

Everything here is based on \cite{BCC+14} (DQL-algorithm) and \cite{KKKW18} (ideas for SGs). 
We first instantiate all macros from Algorithm \ref{alg:BRTDP}.
Note that picking an action from $\best_{\ub,\lb}(last(\path))$ is one of the two things we need to do to extend to SGs. In contrast to the case of MDPs, we are not always interested in the action maximizing $\ub$, but for the minimizing player we use an action that minimizes $\lb$.
For $\GETSUCC$, in the black-box setting there is no choice. We need to sample according to $\trans$, since this is the only way we can learn anything about $\trans$. 

To extend to SGs and to improve the number of steps needed, we change both $\EXPLOREBREAK$ as well as $\HANDLEBEC$. In \cite{BCC+14}, one had to sample for a long time to be acceptably certain that something is an EC, and then the EC was collapsed. 
We change the $\HANDLEBEC$ procedure, to not collapse ECs, but rather to deflate them as in~\cite{KKKW18}. Deflating a set of states is always correct, provided the initial upper bound estimate is correct~\cite[Lemma x]{KKKW18}. Thus, by an inductive argument and Lemma x from \cite{BCC+14}(arxiv), with probability (1- $\delta$) the upper bound estimate is always correct. 
The advantage is, that we do not have to sample for a long time to say that something is an EC with high probability, but we can just deflate any set of states the first time we think it might be an EC. 
This implies that $\EXPLOREBREAK$ can be changed to any reasonable heuristic, e.g. it returns true after the path is longer than $c \cdot \abs{\states}$ for some constant $c \in \Naturals$ or even the first time we see a state twice. We experimentally calculated \todomaxi{Well... last time. Might look at this some more} that setting $c=2$ provides good results.
Also, we cannot make any mistakes in our handling of ECs, in contrast to the collapsing method, where we could only say that with high probability we do something correct.
Here be some description of how deflating works that does not confuse people. Look at Algorithm \ref{alg:ecMDP} for something that probably does not help most people. \textcolor{red}{This is not correct. Two important things: We cannot deflate everything, since in black-box we may not be sure sth is an EC (there might be an action that leaves with a very small prob to target, thus changing value from 0 to 1.) So the algorithm needs to be changed to check, that each action was seen often enough to be kinda sure about its successors, and then it can deflate, which is correct with prob 1-$\delta$ or sth like that. For grey-box, we can just compute restricted game as usual}

\begin{algorithm}[H]
\caption{Procedure for handling end components. Probably we want to handwave this, or we need to go into greater detail and describe restricted game and deflating in more detail.}\label{alg:ecMDP}
\begin{algorithmic}[1]
\Procedure{$\HANDLEBEC$}{upper bound function $\ub$, lower bound function $\lb$, set of states $\Vis$}
\State compute $\G[\Vis]$\label{line:gVis}
\For{$T \in \FIND(\lb,\G[\Vis])$} \label{line:loopAdjust2}
	\State $\ADJUST(T,\ub)$ \label{line:callAdjust2}
\EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}

By changing these two things, picking the next action and how to handle $\CEC$s, we adapted the algorithm to be able to handle SGs, improved the number of steps a simulation needs in the case of ECs and made sure that we never collapse something we are not allowed to collapse.

Now we describe the further improvement we made to the DQL-algorithm, namely changing the $\UPDATE$ procedure.
Algorithm \ref{alg:updMDP} shows the pseudocode of the $\UPDATE$ method. We changed it, so that it does not accumulate the $\ub$- and $\lb$-values, but rather learns the transition probabilities. From those it can calculate the $\ub$- and $\lb$-values in the usual Bellman-equation style. Intuitively, if we have seen a state-action-pair often enough ($m$ times, TBD) to be almost certain about it's probability distribution (with probability 1-$\delta$), we can use it to calculate the estimates of the bounds in every step after that. 
    The advantages are: 
    \begin{itemize}
        \item We do not discard the accumulator after $m$ steps, but keep the information in the learnt probabilities, thereby getting ever more precise estimates of the probabilities over time.
        \item If a $\ub$-value changes, the old algorithm still had the too high value in the accumulator, and could only learn the new value in the next update try. Our algorithm can immediately adjust to new $\ub$-values, since they are not accumulated, but only read during the update.
        \item After seeing a transition $m$ times, we can update the estimates every step after that, in contrast to having to wait for another $m$ steps for the next update.
    \end{itemize}
The general theme here is, that we can be certain of some things or have greater knowledge of some things than before, and then we utilize it (e.g. we are certain deflating is ok, and we can have greater knowledge of transition probabilities and use them, in contrast to learning the possibly changing estimates).

For convenience when writing Bellman updates, we introduce the function $B_f: \states \times \actions \mapsto \Reals$, where $B_f (s,a) = \sum_{s' \in \states} \prob(s,a,s') \cdot f(s')$. Note that it depends on our estimate $\prob$ and not on $\trans$.

This algorithm uses new variables, namely the following:
\begin{itemize}
    \item $m = $ TODO, the number of times we need to see a state-action pair to be approximately certain about its distribution.
    \item $\epsilon_1 = $ TODO, a constant that is added/subtracted in each update of the upper/lower bound estimates to ensure that we stay above/below the true value.
    \item $\epsilon_2$?
    \item $LEARN^{\ub}(s,a)$ and $LEARN^{\lb}(s,a)$, flags that indicate whether the estimates of state-action pair $(s,a)$ may currently be updated. This is only needed for the proof of convergence. TODO: How and when is this set?
    \item $\occ(s,a,s') \in \states \times \actions \times \states \mapsto \Naturals$ counts the number of times a certain triple occurred during all sample trials. It is initialized to 0 for all triples. 
    We use the shorthand $\occ(s,a) = \sum_{s' \in \states} \occ(s,a,s') $ for the number of occurrences of a state-action-pair.
    \item $\prob(s,a,s') \in \states \times \actions \times \states \mapsto [0,1]$ 
    is the current estimate of the probability of a transition from $s$ with action $a$ to $s'$. Note that $\prob$ is only set after a state-action pair has been seen at least $m$ times, so after we are kinda certain that our estimate is good enough.
\end{itemize}




\begin{algorithm}[H]
\caption{Procedure for updating}\label{alg:updMDP}
\begin{algorithmic}[1]
\Procedure{$\UPDATE$}{upper bound function $\ub$, lower bound function $\lb$, path $\path$}
\State $s \gets \pop(\path)$
\Repeat
    \State $t \gets s$ \Comment{Last beginning state becomes target}
    \State $a \gets \pop(\path)$ \Comment{Get state-action pair}
    \State $s \gets \pop(\path)$
    \medskip
    \State $\occ(s,a,t) \gets \occ(s,a,t) + 1$
    \If{$\occ(s,a) \geq m$} 
        \For{$t' \in \states$}
            \State $\prob(s,a,t') \gets \frac{\occ(s,a,t')} {\occ(s,a)}$
            \If {\textcolor{orange}{$LEARN(s,a) \wedge \ub(s,a) - B_{\ub}(s,a) \geq 2 \epsilon_1$}}
                \State $\ub(s,a) \gets B_{\ub(s,a)} + \epsilon_1 $
            \EndIf
            \If {\textcolor{orange}{$LEARN(s,a) \wedge B_{\lb}(s,a) - \lb(s,a) \geq 2 \epsilon_1$}}
                \State $\lb(s,a) \gets B_{\lb(s,a)} - \epsilon_1 $
            \EndIf
        \EndFor
    \EndIf
\Until{$\path$ is empty}
\EndProcedure
\end{algorithmic}
\end{algorithm}





\begin{theorem}
Algorithm \ref{alg:BRTDP}, using Algorithm \ref{alg:updMDP} as $\UPDATE$ and Algorithm \ref{alg:ecMDP} as $\HANDLEBEC$ is PAC, i.e. for any $\epsilon, \delta \in [0,1]$, with probability (1-$\delta$) the Algorithm behaves $\epsilon$-optimal after a number of steps that is polynomial in $\states,\actions,\frac 1 \delta$ and~$\frac 1 \epsilon$.
\end{theorem}
\begin{proof}
We divide the proof into several parts.
\begin{description}
\item We may define some more notation, e.g. $\ub<t>$ for upper bound at time $t$. Maybe we should also say, what exactly a time is. Probably number of iterations of the simulation loop. Also, $\ub[\ast]$ for true upper bound, so value plus $\epsilon_1$.
\item First, assume there are no ECs in the SG. 
\begin{description}
\item Bellman equations unique fixpoint.\\
It follows from \cite{KKKW18}(arxiv) Lemma x and the fact that every BEC is an EC, that then, given an SG $\exGame$ and a combined strategy $\sigma$ \todomaxi{Define this somewhere or drop; how formal do we want to be here?} the system of Bellman equations for the reachability value with the upper bound addition $\epsilon_1$ has a unique fixpoint. 
\item Number of updates bounded.\\
By using the two orange if conditions and the same argumentation as \cite[Lemma 8 and 9]{BCC+14}(arxiv), we know that the number of (successful and attempted) updates of $\ub$ is bounded.
\item If a state is not done and an update of its bounds is attempted, the update succeeds. (The probability that this is violated is bounded by $\delta/6$).\\
Need to change things here. But we can give a bound that $\prob$ is close to $\delta$ since it was sampled for at least $m$ steps, and then, if it is not done, it obviously must succeed in updating.
\item For all timesteps, $\ub<t>(s,a) \geq \val(s,a)$, with probability at least $1-\delta/6$.\\
Can handwave like Strehl and BCC+14, or we really look into that. Sounds believable, that since $\prob$ is close to delta and we have $\epsilon_1$ to guarantee we stay above the true value.
\item If our assumptions hold (which is true with sth depending on $\delta$) and an unsuccessful update occurs, then that state-action-pair is done for the moment.\\
Using what we have before, analogous to Lemma 12 in \cite{BCC+14}. Done for the moment means in $K{t}$, means given the true transition function and the current upper bounds, this pair cannot have a better estimate.
\item The number of timesteps such that a state-action-pair is not done for the moment is bounded.\\
Probably we can even improve the bound, because we only need to see m steps once, and not every time. This is the place for that.
\item Given an SG, a state and the minimal positive transition probability and some $\eta \in [0,1]$, we can find a time $T$ such that 
\[ \val(s) - \val(s,T) \leq \eta\]
i.e. bounded reachability gets us $\eta$ close to the true value.\\
Using Lemma 14 and 15, rather straightforward.
\item Put everything together and juggle numbers, there we have the statement.
\end{description}
\item Now suppose we have an arbitrary SG. 
\begin{description}
\item All bounds stay correct the whole time, as argued in the main body. (Actually, take care of full black-box setting. We might be unlucky and not know that an EC can be left to target and be off by 1. However, this is very unlikely)
\item It remains to prove that there is no EC where we behave suboptimally for more than the allowed number of steps. We follow the proof from \cite[Theorem 2]{KKKW18}(arxiv).
\item Lower bound is not a problem.
\item Assume there was a set of states $X$ where the difference between $\ub$ and $\val$ was greater than $\epsilon$. 
    \begin{description}
    \item It must be a SEC.\\
    There are states not in $X$ (e.g. $\target$ and $\sink$) and by a similar proof to Theorem 1 from \cite{KKKW18}(arxiv) we have that, if it was not a SEC, it would depend on sth on the outside and adjust its value accordingly (with high probability).
    \item We can copy paste steps 9-14 with the exception of taking care of mentioning probabilities everywhere. Idea: There must be a leaving action for maximizer (else everything is deflated to 0; either we have qualitative knowledge, or actually deflate may also do sth wrongly), and at some point minimizers choices are fixed correctly (at least $\epsilon$ correctly, is this a problem?).
    Then there is a best leaving state-action-pair, and then everything is deflated to its value, and hence everything has the value of the best exit, which is a contradiction to the fact that stuff has not converged.
    \item Maybe rewrite to: For every SEC, stuff converges (probably, approximately), and hence everything converges.
    \end{description}
\end{description}
\end{description}
\end{proof}



\iffalse
Note: We need to avoid classifying dummy state as SEC.

\begin{definition}[Restricted game $\mathsf{G}^{X / \states}$]
Let $\exGame$ be an $\SG$ and $X \subseteq \states$.
Then $\exGame[X / \states]$, i.e. the game restricted to $X$, is defined as follows:\todo{less verbose, maybe full thing in appendix}
 \begin{itemize}
\item $\states<\Box>[X / \states] = \states<\Box> \cap X$
\item $\states<\circ>[X / \states] = \states<\circ> \cap X$
\item $\states[X / \states] = \states<\Box>[X / \states] \cup \states<\circ>[X / \states] \cup \set{\dummy}$
\item $\actions[X / \states] = \bigcup_{\state \in X} \Av(\state) \cup \set{\bot}$
\item $\Av[X / \states](\state) = \Av(\state)$ for all $\state \in X$ 

$\Av[X / \states](\dummy) = \bot$
\item $\trans[X / \states](\state,\action) = \trans_\est(\state,\action)$ for all $\state \in X$

The remaining prob goes to $\dummy$ \todo{formal way to write down}
\end{itemize}
\end{definition}
Note that $\dummy$ is a dummy state that has neither a player nor an available action. 
This is against our SG definition. 
But that def was only to classify our input. 
Restricted game is only used for $\FIND$, where dummy does not matter (otherwise it would be special case) and BVI, where we do not include it in the set of updated states (make sure we really do that).
\fi
